NEXT-100 Technical Design Report (TDR). Executive Summary

In this Technical Design Report (TDR) we describe the NEXT-100 detector that will search for neutrinoless double beta decay (bbonu) in Xe-136 at the Laboratorio Subterraneo de Canfranc (LSC), in Spain. The document formalizes the design presented in our Conceptual Design Report (CDR): an electroluminescence time projection chamber, with separate readout planes for calorimetry and tracking, located, respectively, behind cathode and anode. The detector is designed to hold a maximum of about 150 kg of xenon at 15 bar, or 100 kg at 10 bar. This option builds in the capability to increase the total isotope mass by 50% while keeping the operating pressure at a manageable level. The readout plane performing the energy measurement is composed of Hamamatsu R11410-10 photomultipliers, specially designed for operation in low-background, xenon-based detectors. Each individual PMT will be isolated from the gas by an individual, pressure resistant enclosure and will be coupled to the sensitive volume through a sapphire window. The tracking plane consists in an array of Hamamatsu S10362-11-050P MPPCs used as tracking pixels. They will be arranged in square boards holding 64 sensors (8 times8) with a 1-cm pitch. The inner walls of the TPC, the sapphire windows and the boards holding the MPPCs will be coated with tetraphenyl butadiene (TPB), a wavelength shifter, to improve the light collection.

==> src/Radiopurity.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sources of background}

\subsubsection*{Radioactive contaminants in detector materials}

After the decay of \BI, the daughter isotope, \Po, emits a number of de-excitation gammas with energies above 2.3 MeV. The gamma line at 2447 keV, of intensity 1.57\%, is very close to the $Q$-value of \XE. The gamma lines above \Qbb\ have low intensity and their contribution is negligible. 

The daughter of \TL, \Pb, emits a de-excitation photon of 2614 keV with a 100\% intensity. The Compton edge of this gamma is at 2382 keV, well below \Qbb. However, the scattered gamma can interact and produce other electron tracks close enough to the initial Compton electron so they are reconstructed as a single object falling in the energy region of interest (ROI). Photoelectric electrons are produced above the ROI but can loose energy via bremsstrahlung and populate the window, in case the emitted photons escape out of the detector. Pair-creation events are not able to produce single-track events in the ROI. 

\subsubsection*{Radon}
Radon constitutes a dangerous source of background due to the radioactive isotopes $^{222}$Rn (half-life of 3.8\,d) from the $^{238}$U chain and $^{220}$Rn (half-life of 55\,s) from the $^{232}$Th chain. As a gas, it diffuses into the air and can enter the detector. \BI\ is a decay product of $^{222}$Rn, and \TL\ a decay product of $^{220}$Rn. In both cases, radon undergoes an alpha decay into polonium, producing a negative ion which is drifted towards the anode by the electric field of the TPC.  As a consequence, $^{214}$Bi and $^{208}$Tl contaminations can be assumed to be deposited on the anode surface. Radon may be eliminated from the TPC gas mixture by recirculation through appropriate filters. There are also ways to suppress radon in the volume defined by the shielding. Radon control is a major task for a \bbonu\ experiment, and will be of uppermost importance for NEXT-100.

\subsubsection*{Cosmic rays and laboratory rock backgrounds}
Cosmic particles can also affect our experiment by producing high energy photons or activating materials. This is the reason why double beta decay experiments are conducted deep underground. At these depths, muons are the only surviving cosmic ray particles, but 
their interactions with the rock produce neutrons and electromagnetic showers. Furthermore, the rock of the laboratory itself is a rather intense source of \TL\ and \BI\ backgrounds as well as neutrons.

The flux of photons emanating from the LSC walls has been measured \cite{CanfrancFlux}:
\begin{itemize}
\item $0.71 \pm 0.12~{\gamma/\mathrm{cm}^2/\mathrm{s}}$~from the  $^{238}$U chain.
\item $0.85 \pm 0.07~{\gamma/\mathrm{cm}^2/\mathrm{s}}$~from the $^{232}$Th chain.
\end{itemize}

These measurements include all the emissions in each chain. The flux corresponding to the \TL\ line at 2614.5 keV and the flux corresponding to the \BI\ line at 1764.5 keV were also measured (from the latter it is possible to deduce the flux corresponding to the 2448 keV line). The results are:
\begin{itemize}
\item $0.13 \pm 0.01~{\gamma/\mathrm{cm}^2/\mathrm{s}}$~from the \TL\ line.
\item $0.006 \pm 0.001~{\gamma/\mathrm{cm}^2/\mathrm{s}}$~from the \BI\ line at 2448 keV. 
\end{itemize}

The above backgrounds are considerably reduced by the shielding, described in section \ref{sec:Shielding}. In addition, given the topological capabilities of NEXT, the residual muon and neutron background do not appear to be significant
for our experiment. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Radioactive budget of NEXT-100}\label{sec:rabudget}

Information on radiopurity of the materials expected to be used in
the construction of NEXT100 has been compiled, performing specific
measurements and also examining data from the literature for materials
not yet screened. In this executive summary we just present a brief summary, shown in table \ref{tab:RA}, of our detailed database. 

%%%%%%%%%%
\begin{table}
\caption{Activity (in ${\rm mBq}/{\rm kg}$) of the most relevant materials used in NEXT.} \label{tab:RA}
\begin{center}
\begin{tabular}{lllll}
\toprule
Material & Subsystem & Reference &$^{238}$U & $^{232}$Th  \\ \midrule

Lead & Shield & Cometa (supplier) & 0.37 & 0.07 \\

Copper & ICS & Luvata (supplier) & $<0.012$ & $<0.004$ \\

Steel (316Ti) & PV & XENON \cite{Aprile:2011ru} & $<1.9$ & $<1$ \\

Inconel 718 & PV & LSC & $<5.6$ & $<13.8$ \\

Inconel 625 & PV & LSC & $<2.4$ & $<6.0$ \\

Peek & FC/EP/TP & Unizar & 36 & 11.7 \\

Capacitors (Tantalum) & FC/EP/TP & Unizar \cite{ILI1} & 320 & $1.23\times 10^3$ \\

SMD Resistors, Finechem (per pc) & FC & Unizar & 0.022 & 0.048 \\

Polyethylene & FC & XENON \cite{Aprile:2011ru} & 0.23 & <0.14 \\

TTX & LT & ArDM \cite{BOC09}& 12.4 & 1.6 \\

TPB & LT/EP/TP & A. Chemicals \cite{SNOrp} & 1.63 & 0.47 \\
 
PTFE (Teflon) & EP/TP/DB & GERDA \cite{BUD09} & 0.025 & 0.031 \\

PMT (R11410-MOD per pc) & EP & XENON \cite{Aprile:2011ru} & $< 2.5$ & $< 2.5$ \\

PMT (R11410-MOD per pc) & EP & LUX \cite{FAH11}& $< 0.4$ & $< 0.3$ \\

Sapphire window & EP & EXO \cite{LEO08}& 0.31 & 0.12 \\

CUFLON & TP & ICPMS \cite{NIS09}& 0.36 & 0.28 \\

Kapton cable & TP/EP & KAPPA \cite{ILI1} & 14 & 39 \\
\bottomrule
\end{tabular}  
\end{center}
\end{table} 
%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Expected background rate}
NEXT-100 has the structure of a Matryoshka (a Russian nesting doll). The flux of gammas emanating from the LSC walls is drastically attenuated by the lead castle (LC), and the residual flux, together with that emitted by the lead castle itself and the materials of the pressure vessel is further attenuated by the inner copper shielding (ICS). The ICS also attenuates the flux emitted by the tracking plane FE electronics (FEE), which sit behind it. 


One then needs to add the contributions of the ``inner elements'' in NEXT: field cage (FC), energy plane (EP), and the elements of the
tracking plane (TP) not shielded by the ICS.

Thus, the basic ingredients in the NEXT background model recipe are:

\begin{enumerate}
\item The radiation emanating from the Matryoshka, which includes the residual radiation emanating from the LSC walls, from the LC, from the PV and from the FEE, after being attenuated by the ICS.
\item The residual radiation emanating from the ICS, after being attenuated (self-shielding) by the ICS itself.
\item The radiation emanating from the inner elements, namely the FC, the EP and the TP.
\end{enumerate}

As explained above, the only relevant backgrounds for NEXT are the photons emitted by the \TL\ line (2614.5 keV) and the \BI\ line (2448 keV). These sit very near \Qbb\ and the interaction of the photons in the gas can fake the \bbonu\ signal, as we will discuss in the next section.

Our first step, therefore, is to quantify the number of photons crossing the gas emanating from the different sources enumerated above. 

The activity for each material is given in table \ref{tab:RA} in terms of $^{238}$U or  $^{232}$Th decays per unit of time and mass. The high energy photons relevant for NEXT should then be computed by taking into account the branching ratio of the mother nucleus decaying into \BI\ or \TL\  (that is 1 and $\sim 1/3$ respectively), plus the branching ratio of the daughter nucleus itself into the dangerous gamma, plus a geometric factor which reflects the fact that photons coming from nuclear decays are emitted in all directions and not all of them get to reach the gas. The second and the third aspect are included in the rejection factor of background calculated through Monte Carlo (see section \ref{sec:Sensi}). Thus, in the following, the numbers of photons per year are actually the numbers of photons due to a decay of \BI\ or \TL\  (the branching ratio of thorium into thallium is already included), before the correction for the branching ratio and geometric factor. The only exception is the contribution from the LSC walls, which has been measured.


\subsubsection*{Contribution from the Matryoshka}
  
In the following, the contribution to the total activity of each one of the shells of the Matryoshka is described and the photon rates are shown in Table \ref{tab.matrioska}.


The photon flux through the surface of the lead castle is  $4.3\times 10^{10}$  and $9.3\times 10^{11}$ photons per year for \BI\ and for \TL\  respectively. 


The LC is made of radiopure lead. The thickness of the shield is 20 cm and the total mass of the castle is 60 tons, the supplier being most likely COMETA.

The activity of the other components of the lead castle (e.g, external steel support infrastructure) after self-shielding from the lead is negligible compared with the contribution of the lead itself. Notice that the photon rate emitted by the LC is much larger than the residual contribution from the LSC walls in the \BI\ contamination and about the same in \TL. 


The PV is made of radiopure 316Ti alloy and its total mass is 1\,200 kg. We assume
the activity measured by the XENON collaboration (measurements of 316Ti samples are currently under way
at the LSC).
The PV does not act like a shield, but it still respects the Matryoshka principle in the sense that the background rate that it adds is of
the same order of magnitude (actually slightly larger) than the residual background from the outer shell. 
Other elements of the PV such as the Inconel screws add a small contribution. Their specific activity adds a 12.5\% (20\%) extra background rate in \BI\ (\TL) to the PV itself.



The inner copper shield is the most radiopure shell of the Matryoshka. It is made of radiopure copper and its total mass is 1\,200 kg. We consider the activity measured by the supplier (Luvata).The ICS attenuates the radiation coming from the outer shell by two orders of magnitude, and contributes with
a background rate that is almost identical to the residual background. The final rate is
$10^6$ \BI\ photons a year and about one order of magnitude less in \TL.  

\begin{table}
\caption{Number of photons per year outgoing each shell of the Matryoshka. The numbers in bold font are the residual photons after all the shells.}
\label{tab.matrioska}
\begin{center}
\begin{tabular}{lllllll}
\toprule
& \multicolumn{2}{c}{from previous vol after} & \multicolumn{2}{c}{from current vol} &  \multicolumn{2}{c}{total} \\ 
& \multicolumn{2}{c}{passing through current vol} & \multicolumn{2}{c}{(self shielded)} &  \multicolumn{2}{c}{} \\ \midrule
  & \BI\ & \TL\  & \BI\ & \TL\ & \BI\ & \TL\ \\ \midrule
LC & $8.8\times 10^{4}$ & $1.9\times 10^{6}$& $3.2\times 10^{7}$ & $2.1\times 10^{6}$  & $3.2 \times10^{7}$ & $4.0\times 10^{6}$  \\
PV & $1.2 \times10^{7}$ & $1.6\times 10^{6}$ & $4.5\times 10^{7}$ & $7.8\times 10^{6}$ & $5.7\times 1.12\times 10^{7}$ & $9.4\times 1.2\times 10^{6}$ \\
ICS & $5.6\times 10^{5}$ & $9.8\times 10^{4}$ & $5.2\times 10^{5}$ & $5.9\times 10^{4}$ & $\mathbf{1.0\times 10^{6}}$ & $\mathbf{1.6\times 10^{5}}$ \\
\bottomrule
\end{tabular}  
\end{center}
\end{table}


\subsubsection*{Contribution from the inner elements}

The contribution to the total activity from the inner elements is summarized in Table \ref{tab.gtp}.

\begin{table}
\caption{Number of photons per year emitted by the inner elements.}
\label{tab.gtp}
\begin{center}
\begin{tabular}{lcc}
\toprule
   & \BI\ & \TL\  \\ \midrule
TP & $3.2 \times10^{5}$ & $8.2\times 10^{4}$ \\
EP& $8.6 \times10^{5}$ & $2.8\times 10^{5}$ \\
FEE &$7.2\times 10^{5}$ & $5.7\times 10^{5}$ \\
FC & $8.2\times 10^{5}$ & $1.7\times 10^{5}$ \\
\bottomrule
\end{tabular}  
\end{center}
\end{table}


The tracking plane is made of the supporting structure for the DBs (a honeycomb made of PTFE), and the DB themselves, 110 boards made of Cuflon, each weighting about 250 grams. Each DB has 64 MPPCs (glued to the DB with silver epoxy). Each DB has 1 resistor and 2 capacitors. The dominant contribution comes from the DBs themselves, while the addition due to resistors and capacitors is more than two orders of magnitude lower, thus negligible. The contribution of the support structure is also small. 

The energy plane is composed of 60 individual modules plus a vacuum manifold. Each module consists of: (a) one PMT; (b) one PMT base; (c) the can, including its window, support structures, etc. The Hamamatsu R11410-MOD PMTs have been measured by the XENON and the LUX collaborations, and a new measurement is under way at the LSC. Since both measurements are compatible (both are upper limits) we take
the lowest limit (see Table  \ref{tab:RA}). 


The tracking plane front end electronics (FEE) sits behind the ICS and thus its contribution to the
radioactive budget is attenuated by a factor 100. The bulk of the FEE are the 110 front end boards (FEBs). Each FEB will have about 750 resistors and
1100 capacitors. 
The dominant source of background in the field cage is the polyethylene used as an insulator and support of the
field cage rings. The FC support has a mass of 110 kg. The contribution of the metal wires (made of radiopure copper) as well as those of the resistors is negligible compared with that of the polyethylene. 


 
\subsubsection*{Total radioactive budget}
Notice that the leading contribution to the
budget (e.g, in the \BI\ contamination) of the Matryoshka (including LC, PV and ICS), energy plane, field cage and FEE are very similar. An important consequence of this is that a substantial reduction of the radioactive budget can only be achieved if it happens in all the subsystems at the same time. In its current configuration the NEXT radioactive budget is quite balanced. 

The total radioactive budget is $3.7\times 10^6$~photons per year due to \BI\ and  $1.3\times 10^6$~photons per year 
in the \TL\ channel.


==> src/Sensi.tex <==
\subsection{Signal and background characterization in NEXT}

%%%
%\begin{figure}[t!b!]
%\centering
%\includegraphics[width=0.5\textwidth]{img/bb0nu_track_10atm.pdf}
%\caption{\small Double beta decay events have a distinctive topological signature in HPGXe: a ionization track, 
%of about 20 cm length at 15 bar, tortuous because of multiple scattering, and with larger depositions 
%or \emph{blobs} in both ends.}
%\label{fig:track} 
%\end{figure}
%%%

Double beta decay events have a distinctive topological signature in HPGXe (Figure \ref{fig:track}): an ionization track, 
of about 20 cm length at 15 bar, tortuous because of multiple scattering, and with larger depositions 
or \emph{blobs} in both ends. 

As the track propagates in the dense gas it emits $\delta$-rays and bremsstrahlung radiation. Those are typically low-energy gammas with a mean free path below 1 cm. The convolution of emission of electromagnetic energy with the effect of diffusion (about 1 cm for a drift of 1 m) results in a track for \bbonu\ events that looks more like a wiggly, wide "stripe" of energy deposition, about 1-2 cm wide, than like a well defined ``wire'', as usual when tracking high energy muons, for example.  The implications are quite clear:
\begin{enumerate}
\item Space resolution is not an issue in NEXT. A pitch of about 1 cm is sufficient, given the combined effect of
radiation and diffusion, that blur the track into a stripe. Our final design parameter is 1.1 cm.
\item Instead, identification of low energy gammas nearby the track (at distances of a few cm) is important. This is due to the difference between signal (two electrons of average energy \Qbb/2) and the
dominant background (one electron of energy \Qbb). In the second case the probability of radiation is higher and
the mean free path of the gamma is longer. Topologies with one or more isolated clusters of energy, corresponding to
relatively high energy gammas flying distances of 2 or more cm are therefore more likely for the background than 
for the signal. Therefore, identifying low-energy satellite clusters is important in NEXT. This requires a sensor with low energy threshold, as the MPPCs. 
\end{enumerate}


NEXT has three powerful handles to separate \bbonu\ events from backgrounds. These are:
\begin{enumerate}
\item Signal events appear with equal probability in the target, that is, the gas that fills the PV. Defining a fiducial volume, separated from the PV walls by a few cm of active target permits eliminating events in which a high energy gamma is accompanied by charged particles that exit the PV walls. The requirement that the events are strictly contained in the active fiducial volume guarantees that any event with charged activity is eliminated. Notice that, from the point of view of rejecting backgrounds, an HPGXe behaves in a complementary way than a LXe. While liquid xenon has excellent self-shielding properties, xenon gas, even at (moderately) high pressures, is very transparent to gammas.
\item Signal events have all the same energy. Imposing that the events are in the ROI (taken as 0.5\% FWHM) eliminates substantially the backgrounds.
\item Signal events have a distinctive topological signature that can be exploited to further suppress the 
background.  Our calculations yield a rejection factor of 20 at moderate efficiency cost. This is one of the strongest points offered by NEXT
technology.
\end{enumerate}


% ==========================
\subsection{The topological signature} 
\label{sec:sel}

The initial processing of the event allows the ``voxelization'' of the track, which is formed in terms
of connected  3D ``voxels'' formed using the 2D position given by the tracking plane and the
third dimension given by time information. The initial voxels are cubes of 1 cm$^3$~in volume, corresponding 
to the pitch between the MPPCs and twice the EL grid distance. The size of isolated photons is typically one voxel, while a \bbonu\ ``track'' will consist of about 20 voxels. 

An event is accepted as a \bbonu\ candidate if: 
\begin{enumerate}
\item	{\em The event is fully contained in the fiducial volume}
\item	 {\em Only one reconstructed track}: That is the BFS algorithm finds only one connected set of voxels. Events with more than one object (tracks or disconnected voxels) are rejected. 
\item	 {\em Energy in the ROI}: The event is required to be within  1 FWHM  of \Qbb.
\item	{\em \bbonu\ signature}:  the unique track ends in two blobs of high energy, as expected for a \bb\ event. This is translated into a cut $E_{th}=0.4-0.55$~ MeV and $R=2.5-3.0$ cm, that allows a suppression factor between 10 and 20 for the background at the expense of selection efficiency between 78\% and 55\%.
\end{enumerate}
%

To estimate the performance of NEXT-100 \bbonu\ and background data samples have been generated with the NEXUS Monte Carlo simulation. Signal events are simulated in the volume inside the vessel. Backgrounds (\TL\ and \BI\ decays) are simulated in the vessel and in the readout planes. The events thus generated are passed through the selection procedure.  

\begin{table}[t!b!]
\caption{\small Suppression of the \BI\ events by the selection cuts.}
\label{tab:BI}

\begin{center}
\begin{tabular}{cc}
\toprule
Selection criteria & Fraction of events surviving cuts \\ \midrule 
Events analyzed & $10^8$  \\ 
Fiducial, 1 track & $6 \times 10^{-5}$  \\
ROI & $2.2 \times 10^{-6}$  \\ 
Topology & $1.9 \times 10^{-7}$\\ 
\bottomrule
\end{tabular}
\end{center}
\end{table}%


\begin{table}[t!b!]
\caption{\small Suppression of the \TL\ events by the selection cuts.}
\label{tab:TL}
\begin{center}
\begin{tabular}{cc}
\toprule
Selection criteria & Fraction of events surviving cuts \\
\midrule
Events analyzed & $10^8$   \\ 
Fiducial, 1 track & $2.4 \times 10^{-3}$  \\
ROI & $1.9 \times 10^{-6}$  \\ 
Topology & $1.8 \times 10^{-7}$\\ 
\bottomrule
\end{tabular}
\end{center}
\end{table}%

\begin{table}[tb]
\caption{\small Signal efficiency.}
\label{tab:eff}
\begin{center}
\begin{tabular}{cc}
\toprule
Selection criteria & Fraction of events surviving cuts \\ \midrule
Events analyzed & $10^6$   \\ 
Fiducial, 1 track & 0.48  \\
ROI (1 FWHM) & 0.33  \\ 
Topology & 0.25 \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table}%

Tables \ref{tab:BI}, \ref{tab:TL} and \ref{tab:eff} summarize the rejection factors for \BI\ and \TL\ backgrounds as well as the signal efficiency. The background rate of the experiment is obtained  multiplying by the radioactive
budget computed in the previous section.

Multiplying $3.7\times 10^6$~photons per year due to \BI\ by $1.9\times 10^{-7}$~  rejection factor yields 0.7 events
a year in the \BI\ chain. Multiplying $1.3\times 10^6$~photons per year 
due to \TL\ by $1.9\times 10^{-7}$~  rejection factor yields 0.23 events
a year in the \TL\ chain. Thus the expected background number is 1 event a year. 
Divide 1 count by the mass (100 kg) and by the ROI width (12.5 keV) to obtain a
background rate of  $8. \times 10^{-4} \ckky$. If 50 extra kilograms can be found the background rate could
be even lower, $5. \times 10^{-4} \ckky$.

The combination of good resolution, radiopurity and small background rate results in an excellent expected
sensitivity. For a total exposure of 10\,000 $kg\cdot$year (which appears feasible, in particular if we can run
with 150 kg) the sensitivity expected using the PMA NME (\cite{GomezCadenas:2010gs}) is 35 meV, enough
to fully cover the degenerate hierarchy and partially explore the inverse hierarchy. This sensitivity can match or outperform
that of the best experiments in the field. 
  
%%%


==> src/Sensitivity.tex <==


The combination of good resolution, radiopurity and small background rate results in an excellent expected
sensitivity. For a total exposure of 10\,000 $kg\cdot$year (which appears feasible, in particular if we can run
with 150 kg) the sensitivity expected using the PMA NME (\cite{GomezCadenas:2010gs}) is 35 meV, enough
to fully cover the degenerate hierarchy and partially explore the inverse hierarchy. This sensitivity can match or outperform
that of the best experiments in the field. 


==> src/WLSCoating.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Xenon scintillates in the VUV range, with a peak at $\sim$175 nm. On the other hand, the PDE of MPPCs peaks in the blue region and they have a very low PDE below 200 nm. Furthermore the NEXT PMTs will be enclosed in cans coupled to the gas through sapphire windows which are very transparent to the visible light but not to UV (UV grade sapphire is extremely expensive).  Last but not least, the reflectivity of the light tube (made of TTX, a Teflon cloth) is almost 100\% in the visible spectrum and no better than 50\% in the VUV region. 

Consequently, our strategy in NEXT is to shift the VUV light emitted by xenon to the blue region using a wavelength shifter molecule, specifically Tetraphenyl-butadiene (TPB) of $\ge99$\% purity grade. TPB  absorbs light in a wide UV range and re-emits it in the blue with an emission peak around 430~nm.  The molecule can be applied by vacuum evaporation, and other techniques from crystalline form
directly onto surfaces. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{WLS coating of the tracking plane DBs}
A TPB procedure to deposit a thin layer of TPB on flat (relatively small) surfaces, such as daughter boards (DBs) and the sapphire windows of the PMT cans has been developed by the Collaboration \cite{Alvarez:2012ub}. The technique to deposit thin layers in flat surfaces ---including glass, quartz, sapphire and teflon--- has been developed at the coating facility of the Instituto de Ciencias de Materiales (ICMOL).  
Figure~\ref{Fig:evaporator} shows the evaporator used. As an illustration of the procedure, Figure~\ref{Fig:UV_illumination} shows a glass-slice (left) and a prototype DB  (right) coated with TPB and illuminated with UV light at 240~nm,  clearly re-emitting in the blue.
The coated glass-slices and DB samples have been tested and characterized at IFIC and ICMOL with different UV light sources. The procedure and results have been submitted to publication .

%%%%%%%%%%
\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{img/Evaporator2.pdf}
\caption{The evaporator where one can distinguish from bottom to top, the crucibles and the deposition-sensors, the shutter, the sample-holder supported by a spinning disk and the vacuum chamber which is closed down during evacuation and coating.}
\label{Fig:evaporator}
\end{figure}
%%%%%%%%%%

%%%%%%%%%%
\begin{figure}
\centering
\includegraphics[width= 6.5cm]{img/TPB_on_glass2.pdf}
\includegraphics[width= 6.cm]{img/TPB_on_DB.pdf}
\caption{Illumination with 240~nm UV light  of a glass-slice (left) and a 5-SiPM board (right) both coated with TPB.} \label{Fig:UV_illumination}
\end{figure}
%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{WLS coating of the field cage light tube} 
The light tubes will consist of thin sheets of TTX, fixed over a 3M$^{\mathrm{TM}}$.  The TTX will be vacuum coated with TPB. 
 


%%%%%%%%%%
\begin{figure}
\centering
%\includegraphics[width=1.0\textwidth]{img/EvaporatorCollague.pdf}	
\caption{The large evaporation chamber, details.}
\label{fig.chamber}
\end{figure}
%%%%%%%%%%

%%%%%%%%%%
\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{img/FoilTTX.pdf}	
\caption{Response of the light tube foil (ESR+TTX) after coating, showing the characteristic blue
light emission when illuminated by a UV lamp. In the upper part of the picture the same foil without coating.}
\label{fig.foil}
\end{figure}
%%%%%%%%%%

The NEXT collaboration has acquired the large evaporation chamber developed by the ArDM collaboration, which is currently installed at the IFIC (Figure \ref{fig.chamber}).
This is a stainless steel vacuum chamber large enough to house reflector sheets of 120$\times$25~ cm$^2$ which 
have the right size for the NEXT-100 detector. The apparatus consists mainly of two parts, a horizontal tube with pumping connection on its closed end and a slide-in array of 13 crucibles mounted onto a Viton-sealed access flange. The crucibles are electrically connected in series for better uniformity and lower total supply current ($\sim $10A). The reflector sheets are supported by 100$\mu$m wires in a crescent arrangement for constant distance to the crucibles. An evaporation cycle is started by filling the crucibles with TPB powder and positioning the TTX reflector sheet on its support.

After this preparation the sheets were inspected optically with a UV lamp (Figure \ref{fig.foil}) showing the characteristic
re-emission in the blue.

==> src/bkg.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
  
  & U-238 ($\gamma$/year) & Th-232  ($\gamma$/year) \\
\hline
Walls
Lab walls & Canfranc & $5 10^{11}$ & $5 10^{11}$ \\
& & $2 10^7$&    $10^7$ \\
\hline
Pb &     Shield &     &   $5 10^7$&    $ 1.6 10^7$ \\
& & 
\hline

Steel (316Ti) &         PV &    XENON &  <  1.9 &       <   1 \\

Inconel 718 &         PV &        LSC & <5.6 &       < 4.6 \\

Inconel 625 &         PV &        LSC& <2.4 &          <2.0 \\

Peek &   FC/EP/TP &       Unizar &  36 &         11.7 \\

Capacitors (Tantalum) &   FC/EP/TP &   Unizar &      320 &        410 \\

SMS Resistors, Finechem (per pc) &         FC &  Unizar &     0.022 &      0.014 \\

Polyethylene  &         FC &    ELDELWEISS &      16 &       <6 \\
Polyethylene  &         FC &    XENON &      0.23 &       <0.14 \\
Polyethylene  &         FC &    EXO &      < 2.9 &      < 0.57 \\

 TTX &         LT &    ArDM &   12.4 &        1.6 \\

 TPB &   LT/EP/TP &      A. Chemicals & 1.63 &       0.47 \\

PTFE (Teflon) &   EP/TP/DB &      GERDA & 0.025 &      0.031 \\

PMT (R11410-MOD per pc) &         EP &   XENON &    < 2.5 &      <  2.5 \\

PMT (R11410-MOD per pc) &         EP &   LUX &    < 0.4 &      <  0.3 \\

Sapphire window &         EP &    EXO &   0.31 &       0.12 \\

    CUFLON &         TP &   ICPMS &    0.36 &       0.28 \\

Kapton cable &      TP/EP &   KAPPA &      14 &         13 \\
\hline\hline
\end{tabular}  
\caption{Activity of the most important materials used in NEXT. The numbers are selected from
the detailed repot available at the NEXT web page.}
\label{tab:RA}
\end{center}
\end{table} 



==> src/rpty.tex <==
\begin{table}[tb]
\caption{Activity (in mBq/kg) of the most important materials used in NEXT. The numbers are selected from the detailed report available at the NEXT webpage.} \label{tab:RA}
\begin{center}
\begin{tabular}{lllll}
\toprule
  Material & NEXT system & Reference &$^{238}$U & $^{232}$Th  \\
\hline
%%        Pb &     Shield &    Mifer (supplier) &   0.33 &        0.1 \\
         Pb &    Shield &    Cometa (supplier) &   0.37 &        0.07 \\

        Cu &        ICS &    Luvata (supplier)  & <0.012 &    <  0.004 \\

Steel (316Ti) &         PV &    XENON \cite{Aprile:2011ru} &  <  1.9 &       <   1 \\

Inconel 718 &         PV &        LSC & <5.6 &       < 13.8 \\

Inconel 625 &         PV &        LSC& <2.4 &          <6.0 \\

Peek &   FC/EP/TP &       Unizar &  36 &         11.7 \\

Capacitors (Tantalum) &   FC/EP/TP &   Unizar \cite{ILI1} &      320 &        $1.23\times 10^3$ \\

SMD Resistors, Finechem (per pc) &         FC &  Unizar &     0.022 &      0.048 \\

Polyethylene  &         FC &    XENON \cite{Aprile:2011ru} &      0.23 &       <0.14 \\

 TTX &         LT &    ArDM \cite{BOC09}&   12.4 &        1.6 \\

 TPB &   LT/EP/TP &      A. Chemicals \cite{SNOrp} & 1.63 &       0.47 \\
 
PTFE (Teflon) &   EP/TP/DB &      GERDA \cite{BUD09} & 0.025 &      0.031 \\

PMT (R11410-MOD per pc) &         EP &   XENON \cite{Aprile:2011ru}  &    < 2.5 &      <  2.5 \\

PMT (R11410-MOD per pc) &         EP &   LUX \cite{FAH11}&    < 0.4 &      <  0.3 \\

Sapphire window &         EP &    EXO  \cite{LEO08}&   0.31 &       0.12 \\

    CUFLON &         TP &   ICPMS \cite{NIS09}&    0.36 &       0.28 \\

Kapton cable &      TP/EP &   KAPPA  \cite{ILI1}&      14 &         39 \\
\bottomrule
\end{tabular}  
\end{center}
\end{table} 



==> src/screening.tex <==
\subection{Control of material radiopurity}

Information on radiopurity of the materials expected to be used in
the construction of NEXT100 has been compiled, performing specific
measurements and also taking data from the literature for materials
not yet screened. In this executive summary we just present a brief summary. 
A much more detailed information can be found online at:
\begin{itemize}
\item \url{http://next.ific.uv.es/next/}
\end{itemize}

\input{src/rpty.tex}


